Scalable, Validated Code Translation of Entire Projects using Large Language Models

Large language models (LLMs) show promise in code translation due to their ability to generate idiomatic code. However, a significant limitation when using LLMs for code translation is scalability: existing works have shown a drop in translation success rates for code exceeding around 100 lines. We overcome this limitation by developing a modular approach to translation, where we partition the code into small code fragments which can be translated independently and semantically validated (that is, checking I/O equivalence). When this approach is applied naively, we discover that LLMs are unreliable when translating features of the source language that do not have a direct mapping to the target language, and that the LLM often gets stuck in repair loops when attempting to fix errors. To address these issues, we introduce two key concepts: (1) feature mapping, which integrates predefined translation rules with LLM-based translation to guide the LLM in navigating subtle language differences and producing semantically accurate code; and (2) type-compatibility, which facilitates localized checks at the function signature level to detect errors early, thereby narrowing the scope of potential repairs. We apply our approach to translating real-world Go codebases to Rust, demonstrating that we can consistently generate reliable Rust translations for projects up to 6,600 lines of code and 369 functions, with an average of 73% of functions successfully validated for I/O equivalence, considerably higher than any existing work.

==> aux.tex <==
\paragraph{Our type consistency checks catch translation errors otherwise missed by the Rust compiler} \autoref{fig:go_snippet_semantics} presents a \textcolor{Go}{Go} snippet we extracted from the \textbf{ach} benchmark. The data structure \gocode{EntryDetail} contains a nullable \textcolor{Go}{Go} slice \gocode{[]*Addenda05}. The function \gocode{addendaFieldInclusion} receiving an argument \gocode{entry} of type \gocode{EntryDetail}, performs a null check on the \gocode{Addenda05} field.

\begin{figure}[!htb]
    \centering
    \begin{minipage}{.5\textwidth}
        % \centering
        \begin{lstlisting}[language=go, basicstyle=\tiny\ttfamily]
type EntryDetail struct {
	Addenda05 []*Addenda05
}
func (batch *Batch) addendaFieldInclusion(entry *EntryDetail) error {
    if entry.Addenda05 != nil {
        return batch.Error(...)
    }
    ...
}
\end{lstlisting}
        \caption{Source Go snippet}
        \label{fig:go_snippet_semantics}
    \end{minipage}%
    \begin{minipage}{0.5\textwidth}
        % \centering
        \begin{lstlisting}[language=rust, basicstyle=\tiny\ttfamily]
pub struct EntryDetail {
    pub addenda05: Vec<Option<Box<Addenda05>>>,
}
pub fn addenda_field_inclusion(&self, entry: &EntryDetail) -> Result<()> {
    if entry.addenda05.iter().any(|a| a.is_some()) {
        self.error(..)?;
    }
    ...
}
\end{lstlisting}
        \caption{Translated Rust snippet}
        \label{fig:rust_snippet_semantics}
    \end{minipage}
\end{figure}

\autoref{fig:rust_snippet_semantics} is the \textcolor{Rust}{Rust} translation we obtained from LLMs. Note that nullability is missing as \rustcode{Vec<Option<Box<Addenda05>>>} is a non-null object. However, LLMs manage to generate a compilable translation for the function, which instead checks if any entry into \rustcode{entry.addenda05} is null. 
%
While the resulting translation passes the Rust compiler, it does not reflect the same intent as the original code. 
Conversely, our type consistency checks catch this translation error as a null value can inhabit
the \gocode{Addenda05} field
of \gocode{EntryDetail}, whereas this in not possible in the Rust translation.
=============

\paragraph{Our type compatibility checks are local, enabling us to catch type errors early on} 
If we consider the example in~\autoref{fig:go_snippet_compilation} taken from the realworld benchmark \textbf{ach}, function \gocode{GetControl} returns a nullable object, for which its caller, \gocode{IsADV}, performs a null-check. \autoref{fig:rust_snippet_compilation} contains a \textcolor{Rust}{Rust} translation obtained from LLMs. Note that, conversely to the original code, the return of function \gocode{get\_control} cannot be null. Given that LLMs tend to emulate the syntax of the source code, the null-check for the result of \rustcode{get\_control} is translated as is despite the fact that \rustcode{get\_control} cannot return null. While this does cause a compilation error, such an error is only generated after the callee \rustcode{is\_adv} has been translated, causing the overall translation process to backtrack and re-query the LLM for \rustcode{GetControl}. Conversely, our type consistency checks are able to catch this error at the point where \gocode{GetControl} is translated.

\begin{figure}[!htb]
    \centering
    \begin{minipage}{.5\textwidth}
        % \centering
        \begin{lstlisting}[language=go, basicstyle=\tiny\ttfamily,escapechar=\&]
func (batch *Batch) GetControl() *BatchControl {
	return batch.Control
}
func (f *File) IsADV() bool {
    for i := range f.Batches {
        if v := f.Batches[i].GetControl(); v == nil {
            ...
        }
        ...
    }
    ...
}
&\newline&
&\newline&
&\newline&
&\newline&

\end{lstlisting}
        \caption{Source Go snippet}
        \label{fig:go_snippet_compilation}
    \end{minipage}%
    \begin{minipage}{0.5\textwidth}
        % \centering
        \begin{lstlisting}[language=rust, basicstyle=\tiny\ttfamily]
impl Batch {
     fn get_control(&self) -> &BatchControl {
        &self.control.as_ref().unwrap()
    }
}
impl File {
    pub fn is_adv(&mut self) -> bool {
        for batch in &mut self.batches {
            if batch.get_control().is_none() {
                ...
            }
            ...
        }
        ...
    }
}
\end{lstlisting}
        \caption{Translated Rust snippet}
        \label{fig:rust_snippet_compilation}
    \end{minipage}
\end{figure}
==========

\begin{minipage}{.45\textwidth}
        % \centering
        \begin{lstlisting}[language=rust, basicstyle=\tiny\ttfamily,escapechar=\%]
pub fn update_ranks(ranks: &mut Rank, algorithm: &dyn Algorithm) {
    todo!()
}
%\newline%
%\newline%
%\newline%
%\newline%
%\newline%
\end{lstlisting}
        \caption{Bypassing the Rust compiler check}
        \label{fig:rust-bypass}
    \end{minipage}%

==> imports.tex <==
\section{Generating the project layout and visibility modifiers}
%So far we have considered code generation within single file. 
Real-world \textcolor{Go}{Go} projects have their source code distributed into a complex project layout. 
%Meanwhile, those projects often rely on 3rd party libraries. For simplification, we limit our scope to project consists of a single package. For idiomaticity, we need to keep the same file structure in the translation and use appropriate 3rd party libraries in \textcolor{Rust}{Rust}.
The challenge in translating such projects arises from the different code organization principles of
\textcolor{Go}{Go} and \textcolor{Rust}{Rust}. A \textcolor{Go}{Go} project consists of packages, where a package can span multiple files. Private items are visible to other items in the same package, even if they are not in the same file. Conversely, \textcolor{Rust}{Rust} obeys a module system,  where each file in a \textcolor{Rust}{cargo} project is a module. Items in a module cannot be directly used by items in another module. 

Relying on the LLM to make decisions on the project structure and appropriately generate import statements and amend visibility modifiers is problematic. 
In fact, Yin et al. found that the most frequent compilation errors for code obtained through LLM-based translation are related to wrong or missing import statements~\cite{yin2024rectifiercodetranslationcorrector}.


%However, keeping complex file structure can bring various compilation issues related to wrong/missing import statements~\cite{yin2024rectifiercodetranslationcorrector}, which is contribute to a major proportion of compilation errors in project translation. We discuss two kinds of wrong/missing import statements.

\paragraph{Internal imports.} %\textcolor{Go}{Go} and \textcolor{Rust}{Rust} have different code organization principles. A \textcolor{Go}{Go} package can be defined by multiple files. Private items are visible to other items in the same package, even if they are not of the same file. \textcolor{Rust}{Rust} obeys a module system,  where each file in a \textcolor{Rust}{cargo} project is a module. References of items in another module necessitate an internal import statement to explicit state which item to use from what module. 
Our approach is to emulate the original project structure.
For this purpose, we symbolically generate the appropriate import statements by using our dependency analysis, and amend the translated code accordingly as part of post-processing.

%The mechanization of internal import statement generate does not only improve reliability of the generated code, but also simply the prompt design: we are able to hide the complex file structure to the LLMs.

\paragraph{External imports.} Translation of \textcolor{Go}{Go} projects with 3rd party dependencies is challenging because we either need to translate the entire library, or we must find appropriate \textcolor{Rust}{Rust} libraries that have the same functionality as their \gocode{Go} counterpart.
Our solution is to rely on the LLM to find appropriate third-party library mappings and generate corresponding external import statements.  Our experience is that, owing to their large training sets, LLMs are frequently able to identify suitable third party Rust libraries.


%In the Go code shown in \autoref{fig:go_overview}, where all the files are in the same package, all items are accessible to one another due to Go's visibility rules. By contrast, Rust defaults to private visibility, where items are only accessible within the same module (i.e. file in our case). Rather than depending on the LLM, we symbolically generate the appropriate visibility modifiers for the Rust translation, as demonstrated in Figure~\ref{fig:rust_overview_correct}, where \rustcode{pub} is added to make items public where appropriate.


==> intro.tex <==
\section{Introduction}
The task of translating programs between languages is becoming increasingly essential due to the growing interest in safe programming languages like Rust and the need to convert legacy code into these modern, reliable languages~\cite{tractor}. 

Current methods for automatically translating to Rust generally fall into two categories: symbolic (i.e. rule-based)~\cite{} and relying on Large Language Models (LLMs)~\cite{}. Symbolic methods make use of static analysis to predefine conversion rules, which are crafted to be sound and can often scale 
to real-world codebases ~\cite{zhang2023ownership}. 
%\cd{mention numbers for LoC?}
%so that a single, global pass over an entire project 
%resulting in correct-by-construction translations. 
As a downside, such approaches often produce non-idiomatic and unsafe Rust code~\cite{}. This limits their practical usability, as the resulting code can be difficult to maintain and may retain the same safety risks as the original code. 

Conversely, LLM-based translation generates more idiomatic and safer Rust code, reducing reliance on unsafe constructs and improving maintainability. However, a significant limitation of this class of approaches is scalability; existing works have shown a drop in translation success rates for code exceeding around 100 lines~\cite{eniser2024translatingrealworldcodellms}, rendering the translation of large-scale, real-world projects impractical with current methods.

The challenges of scaling translation are many-folds. Firstly, the limited size of context windows of LLMs necessitates modular translation, demanding code partition of the source code repository; secondly, disparate source and target language features may frustrate code compilation and there is a lack of clear definition of translation correctness; thirdly, LLMs often suffer from hallucinations, obliging response filtering/code corrections based on formal analysis.

Our goal is to combine the strengths of the two approaches by leveraging 
rule-based translation and static analysis to scale LLM-based translation to real-world code. We illustrate our technique
in the context of translating Go to Rust.

\paragraph{Features Mapping} We propose a novel concept called \emph{features mapping} that defines high-level code translation rules to constrains code-generation by LLMs. When there are small syntactic or semantic differences between constructs in the source and target languages, LLMs may incorrectly emulate the syntax of the source language, or wrongly map source
APIs to target ones, leading to code that does not properly compile or doesn't maintain the behavior of the original code~\cite{yin2024rectifiercodetranslationcorrector}.
%
This ranges from basic features (e.g. variable definitions, struct definitions) to more involved ones such as interface declarations and error handling. Our observation is that, while getting these features correct is challenging for the LLM, a rule-based approach can easily match the source and target features. Specifically, features mapping partition the source program into individual units categorized by source language features. For each source language feature, we pre-defined a target language feature and a prompt-template that query for the target feature. Finally, we invoke syntactic checks to filter out code with bad features and automatically amend code towards the desired target features.

\paragraph{Incremental Translation Correctness} Based on features mapping, we formally define translation correctness to enable step-by-step code validation. Specifically, by borrowing ideas from multi-language semantics/language interoperability community, we define a two-language semantics for source/target features using data marshaling. We construct oracles to check semantics equivalence at each step.

\paragraph{Project Sketch Construction}

\paragraph{Iterative Refinement}\hlz{Not sure if we should add this}



==> intro_old.tex <==
\section{Introduction}\label{sec:intro}

The task of translating programs between languages is becoming increasingly essential due to the growing interest in safe programming languages like Rust and the need to convert legacy code into these modern, reliable languages~\cite{tractor}. 

Current methods for automatically translating to Rust generally fall into two categories: symbolic (i.e. rule-based)~\cite{} and relying on Large Language Models (LLMs)~\cite{}. Symbolic methods make use of static analysis to predefine conversion rules, which are crafted to be sound and can often scale 
to real-world codebases ~\cite{zhang2023ownership}. 
%\cd{mention numbers for LoC?}
%so that a single, global pass over an entire project 
%resulting in correct-by-construction translations. 
As a downside, such approaches often produce non-idiomatic and unsafe Rust code~\cite{}. This limits their practical usability, as the resulting code can be difficult to maintain and may retain the same safety risks as the original code. 

Conversely, LLM-based translation generates more idiomatic and safer Rust code, reducing reliance on unsafe constructs and improving maintainability. However, a significant limitation of this class of approaches is scalability; existing works have shown a drop in translation success rates for code exceeding around 100 lines~\cite{eniser2024translatingrealworldcodellms}, rendering the translation of large-scale, real-world projects impractical with current methods.

%This is due to the fact that the size of real-world projects is likely to exceed the LLM's context window. Even if the token limit allows translating a project in a single pass, existing works have reported a degradation in the LLMs' reasoning performance at much shorter input lengths than their technical maximum~\cite{DBLP:conf/acl/LevyJG24}.

%Consequently, the initial translation is unlikely to be fully correct. 
%Verifying translations as well as diagnosing and resolving errors in large codebases, is particularly challenging when approached globally. Research in software verification generally addresses this complexity through modularity, breaking down tasks into manageable units.

Our goal is to combine the strengths of the two approaches by leveraging static analysis and rule-based translation to scale LLM-based translation to real-world code. We illustrate our technique in the context of translating Go to Rust \cd{motivation for this?}.

\paragraph{Partitioning the code into smaller units that can be translated modularly}
A natural approach to improving the scalability of LLM-based translation is to partition the code into smaller units, and then translating them individually. 
%independently of the rest of the project. 
Following this strategy, we partition the code at function boundaries in order to translate each function separately, beginning with callees and then callers. When translating a function, we populate the prompt's context with relevant information about data types, callees, and global elements. After obtaining a translation, we verify its correctness. If the translation is correct, we proceed to the next function; if not, we requery the LLM to address the flagged error. 

The problem with this naive approach is that a function's translation may not integrate well with the rest of the project, causing the correctness check to raise errors in already translated and validated parts of the project. As an example, during a function's translation, the LLM may decide to change the signature of one of its callees, which will trigger a compilation error.
This requires backtracking and requerying the LLM to correct faulty dependencies, including any previously translated functions that rely on them. Such a situation presents a significant challenge, making it impossible to predict the overall progress of the translation process.

The core issue lies in the LLM's unconstrained freedom to modify the project at each translation step, compounded by the global correctness checks. In order to address these issues, we apply two main strategies.

%In order to make LLMs scale to real-world projects, we need more than code partitioning.
%Next, we make use of static analysis  and rule-based translation to constrain the LLM's scope in terms of what code it can generate and when. %The overall goal is to prune the search space in LLM-based translation, thus enhancing scalability.
 %We discuss these techniques next.

%Thus, we combine symbolic and LLM-based reasoning to prune the search space.

%The complex dependencies involving real-world projects make their translation and verification inherently non-modular. In this paper, we attempt to improve scalability with the following techniques:

\paragraph{\textbf{Strategy 1: Use static analysis and rule-based translation to constrain the code generated by the LLM}}
Next, we discuss two use cases of this strategy.
%Feature mapping between the source and target projects.
\paragraph{A. We propose rule-based feature mapping that defines high-level
code translation rules to avoid mistakes commonly made by LLMs}
%LLMs make mistakes that can be easily avoided by rule-based methods
%LLMs may miss differences between language features.
When there are small syntactic or semantic differences between constructs in the source and target languages, LLMs may incorrectly emulate the syntax of the source language, or wrongly map source
APIs to target ones, leading to code that does not properly compile or doesn't maintain the behaviour of the original code~\cite{yin2024rectifiercodetranslationcorrector}.
%
This ranges from basic features (e.g. variable definitions, struct definitions) to more involved ones such as interface declarations and error handling. Our observation is that, while getting these features correct is challenging for the LLM, a rule-based approach can easily match the source and target features. 
We statically analyse the original code to detect features of interest, and then apply symbolic rules to instruct the LLM on the corresponding features in the target translation. 
%

\paragraph{B. We use static analysis to determine the project layout}

%Real-world \textcolor{Go}{Go} projects often consist of multiple packages, with source code organized in a complex project layout.  
The challenge arises from the different code organization principles of
\textcolor{Go}{Go} and \textcolor{Rust}{Rust}. A \textcolor{Go}{Go} project consists of packages, where a package can span multiple files. Private items are visible to other items in the same package, even if they are not in the same file. Conversely, \textcolor{Rust}{Rust} obeys a module system,  where each file in a \textcolor{Rust}{cargo} project is a module. Items in a module cannot be directly used by items in another module. Relying on the LLM to make decisions on the project structure and appropriately generate import statements and amend visibility modifiers is problematic. 
In fact, Yin et al. found that the most frequent compilation errors for code obtained through LLM-based translation are related to wrong or missing import statements~\cite{yin2024rectifiercodetranslationcorrector}.
Our approach is to emulate the original project structure, and use a dependency analysis to statically synthesise the correct import statements and visibility modifiers. 



\paragraph{\textbf{Strategy 2: Perform incremental verification of the translation that prioritises local checks over global ones in order to limit LLM re-querying}}
%the LLM's ability to modify already translated parts of the project}
As previously mentioned, one of the issues we are trying to address is the need to revisit and re-query the LLM for already translated and validated parts of the project.
For this purpose, we divide the translation process into two phases: type-driven and semantics-driven, where only the former is allowed to perform such re-querying. The type-driven phase aims to generate a \emph{type-correct project sketch}, which is a project that compiles and follows specific type equivalence rules relative to the original project, though it may not yet be semantically equivalent. Notably, the custom type equivalence rules are local, as opposed to the compiler check, which is global. 
%For this purpose, we make extensive use of Rust's type system to identify as many integration errors as possible. In addition to relying on the Rust compiler, we implement extra type checks that relate types in the original and target code (detailed later in the paper). Backtracking is permitted during this phase.

The semantics-driven phase focuses on establishing semantic equivalence with the original project. Here, we make the assumption that the project sketch generated during the type-driven phase is indeed type-correct, and disallow the LLM from modifying any type-related information (e.g. function signatures). Additionally, we restrict the correctness check 
to focus solely on local errors within the current function by creating mocks of its callees that emulate their behavior in the original code. The consequence of these two constraints is that backtracking, and therefore re-querying the LLM for parts of the project that were already translated and validated, is never required.

%, without the option to backtrack. Essentially, each function is checked for semantic equivalence and repaired independently of the rest of the project. 
%One consequence is that, even though we may not be able to find a translation that is fully semantically equivalent to the original, the transtion will terminate with a partially correct one.


%\cd{clarify the scope}
%We are interested in translating large real-world Go projects to Rust \cd{motivate?}.   

\paragraph{Contributions} \cd{in progress..}
\begin{itemize}
    \item We propose techniques for improving the scalability of LLM-based translation to Rust.
    \item We make use of Rust's type system to generate type-correct project sketches and constrain the search performed by the LLM.
    \item We make use of rule-based methods to match features between the original and target code, thus avoid mistakes commonly made by LLMs.
    \item We implemented our design and used it to translate four open-source Go projects to Rust. \cd{more details about the results}
\end{itemize}

==> old_notes.tex <==
\section{Differences in Language Features}
Beyond basic language features like functions, global variables, constants, realistic software are often composed by using language constructs like methods, interfaces, classes, traits, etc. Those constructs are often unique to a particular language; syntactically similar constructs in different languages may be incompatible to each other (e.g. Go interfaces and Rust traits). However, LLMs tend to emulate the source language syntax~\cite{yin2024rectifiercodetranslationcorrector}, resulting in sub-optimal decisions. Specific instructions are thereby required to guide the code generation process.

% We propose to apply specialised prompts or automatic corrections to aid the translation.

\subsection{Go Interface}

Take the following Go interface with two methods as an example,
\begin{lstlisting}[language=go]
type I interface {
    func method1()
    func method2()
}
\end{lstlisting}
To implement this interface for a type \lstinline{T}, the programmer needs to provide concrete definitions for those two methods, \emph{separately}.
\begin{lstlisting}[language=go]
func (T t) method1() {
    ...
}
func (T t) method2() {
    ...
}
\end{lstlisting}

Similar concepts (traits) exist in Rust,
\begin{lstlisting}[language=rust]
trait I {
    fn method1(&self);
    fn method2(&self);
}
\end{lstlisting}
But this time, to implement traits for a type \lstinline{T}, one would need to provide all definitions \emph{together} in an impl-block.
\begin{lstlisting}[language=rust]
impl I for T {
    fn method1(&self) { ... }
    fn method2(&self) { ... }
}
\end{lstlisting}

When doing modular translation at the function-level, we observed that LLMs are able to generate the correct correspondence between the Go interface definition and the Rust trait definition, but struggle to generate the correct correspondence between methods implementations, even if we provide the information that those methods belong to an interface in the prompt. This is very intuitive as LLMs have no idea of \lstinline{method2} when translating \lstinline{method1}, and that both translations are required to be put in one impl-block.

Our idea is to pre-define a set of \emph{feature-mappings} which essentially ``teach" the LLMs how to deal with advanced language  features. In the above example, a tentative solution is to break down the Rust trait into multiple sub-traits,
\begin{lstlisting}[language=rust]
trait I1 {
    fn method1(&self);
}
trait I2 {
    fn method2(&self);
}
trait I: I1 + I2 {}
impl<T: I1 + I2> I for T {}
\end{lstlisting}
Now any types that implement both sub-traits will automatically implement trait \lstinline{I}, which corresponds to the original interface.
When translating \lstinline{method1}, we instruct the LLMs specifically that it should put the Rust method in the following block,
\begin{lstlisting}[language=rust]
impl I1 for T {
    ...
}
\end{lstlisting}
This approach allows us to query the translation of \lstinline{method1} independently of \lstinline{method2}, implying modularity.

% \subsection{Error Handling}
% Compared to Go programs, Rust programs handle errors differently in the following ways:

% \emph{Error representation.} In Go, the built-in \lstinline{error} type defines an interface with a single method, \lstinline{Error() string}, which converts the error value to a string; in Rust, the standard library provides the \lstinline{std::error::Error} trait, but it depends on the \lstinline{std::fmt::Display} trait to implement the string conversion method.

% \emph{Handling mechanism. }
% The Go language adopts C-style error handling, where a fallibale function returns, in addition to its result, an explicit \lstinline{error} value. Whereas in Rust, such function returns a \lstinline{Result} enum to represent success or failure.

% We observed that LLMs are capable of converting handling mechanisms, but struggles with converting error representations.

\subsection{Java Classes}
A Java class file consists of a class definition, which
includes field definitions, static variables, constructors, methods and static methods. A naive translation (which LLMs often do) is to generate a Rust struct which includes all fields, and represent all other
items as associated methods, as shown in the following,
\begin{lstlisting}[language=java]
public class Factory {
    public Factory() { /* ... */ }
    public Widget produceWidget() { /* ... */ }
    public void consumeWidget(widget w) { /* ... */ }
}
\end{lstlisting}
is translated to
\begin{lstlisting}[language=rust]
pub struct Factory {
    /* ... */
}

impl Factory {
    pub fn new() -> Factory { /* ... */ }

    pub fn produce_widget(&self) -> Widget { /* ... */ }

    pub fn consume_widget(&self, widget: Widget) { /* ... */ }
}
\end{lstlisting}
This style of translations works for a single class file, but struggles with classes with extensions: if a
class \lstinline{C} extends \lstinline{Factory}, then
\begin{enumerate}
    \item What type should \lstinline{C} be mapped to? Should it be a struct that contains \lstinline{Factory} as a field?
    \item The methods \lstinline{produce_widget} and \lstinline{consume_widget} should be available to \lstinline{C} because of inheritance, how shall this be reflected in Rust translations?
\end{enumerate}

There are some other concerns on how to translate overloaded functions (namely, functions with the same name but different arguments), which is not supported in Rust.
In our prior experiments, we noticed that Java benchmarks have low compilation rate due to these unsupported features.

% I've found a library dedicated for Java-Rust interoperation\footnote{\href{https://duchess-rs.github.io/duchess/call_java_from_rust.html}{Duchess}}, which translates a class definition in the following way,
% \begin{lstlisting}[language=rust]
% // One struct per Java class:
% pub struct Factory { /* ... */ }

% // The inherent impl defines the constructor
% // and any static methods:
% impl Factory { /* ... */ }

% // The extension trait defines the methods
% // on the struct, like `produceWidget`
% // and `consumeWidget`.
% pub trait FactoryExt { /* ... */ }
% \end{lstlisting}
% My understanding is that putting methods in an extension trait can help with inheritance.


% \subsection{Go Type Embedding}
% Go has a unique language construct called type embedding,
% \begin{lstlisting}[language=go]
% type A struct {
%     G string
% }
% type B struct {
%     F int
%     A
% }
% \end{lstlisting}
% In the above code snippet, struct \lstinline{B} is built by including \lstinline{A} directly.
% The quirk is that, as a syntactic sugar, a \lstinline{B} object can use all methods of \lstinline{A}.

% We observed that LLMs 


\subsection{File Structure and Visibility}
Programs in modern languages are often structured with file hierarchies for code maintenance, item visibility for abstraction, and other organisational principles. These principles often differ across languages, necessitating specialized prompts or automatic corrections.

\subsection{Misc. Specific Instructions}
\subsubsection{Error Type Representation} Go programs often use the built-in \lstinline[language=go]{error} interface type to represent an error value. Rust has a similar concept with the \lstinline{Error} trait from the standard library. However, since the latter isn't a type, there is no direct correspondence between the two. And in fact, we observed that LLMs struggles with translating Go error types: they generate non-compilable code or map Go \lstinline[language=go]{error} to concrete error types, resulting in inconsistent code. Our solution is to instruct LLMs to use a Rust 3rd party library (anyhow~\footnote{\hyperlink{https://crates.io/crates/anyhow}{anyhow}}) which provides an error type that resembles the Go \lstinline[language=go]{error} interface.

\subsubsection{Variadic Arguments} Rust doesn't support variadic arguments. We noticed that LLMs generate code that doesn't compile (e.g. use an \lstinline{Any} type to represent variadic arguments). A tentative solution is to instruct the LLMs to generate a function with a vector as argument which corresponds to the original variadic arguments.




\section{Translation Order}
Real-world projects are often composed of deeply interconnected components: a function may reference a set of other functions, constants, global variables and types. When querying the translation of a function, we need to either query the used items on demand or predefine a translation order so that translations of all used items are already available. As a result, we have two algorithms:

\emph{On-demand.} We follow the postorder of the callgraph, starting from the bottom-level functions. Whenever there are used types/constants/global variables not translated but used in the current function, we query their translations along with the function translation.

\emph{Prescheduled.} Translations are performed in multiple phases. In the first phase, we translate all types following the postorder of the type-dependency graph; in the second phase, we translate all constants; in the third phase, all global variables; in the final phase, all functions in postorder of the callgraph.

The advantage of the on-demand algorithm is that functions serve as natural \emph{usage examples} for types/constants/globals variables so that the LLMs can potentially make better decisions. However, we might need a better translation order than postorder of the callgraph. Consider the following scenario: function \lstinline{f} uses type \lstinline{A} (by accessing one field of it), which internally references type \lstinline{B}; function \lstinline{g} uses type \lstinline{B} only; suppose further that \lstinline{g} and \lstinline{f} are both leaves functions in the callgraph, thus postorder cannot distinguish between them. 

In this scenario, we need to query translations for both \lstinline{A} and \lstinline{B} on the fly when translating \lstinline{f} even if \lstinline{f} does not use \lstinline{B} at all (the field accessed by \lstinline{f} has nothing to do with \lstinline{B}, so the LLM will have little information about \lstinline{B}). Therefore, it would be better if we start from \lstinline{g} instead of \lstinline{f}.

The advantage of the pre-scheduled algorithm is that the implementation is simple. However, we might need to provide usage examples when translating types.

\hlz{Currently we are following the prescheduled algorithm because it's simpler.}

\section{A Backtracking Translation Loop}
Our modular algorithm queries translations in a specific order, aborting if it fails to find a compilable translation for the current item. However, we have frequently observed that these failures often stem from an earlier translation step. For instance, a function's callee might be translated into a compilable Rust function, but its type signature may not be compatible with the current function. This motivates a backtracking translation algorithm, which analyzes the compilation error message and calculates an appropriate translation step to backtrack to.

==> overview.tex <==
\section{Overview of our approach}
%\cd{revise and use running example}
%We construct a call-graph, which we then traverse in post-order, and translate each individual function.
We illustrate our approach using the example in Figure~\ref{fig:go_overview}, which is a slightly contrived version of code extracted from the realworld benchmark \textbf{ach}. 
%
The example features a data structure \gocode{EntryDetail} containing a nullable \textcolor{Go}{Go} slice \gocode{[]*Addenda05},
a function \gocode{checkAddenda02} and a method
\gocode{addendaFieldInclusion}.

\paragraph{Project partitioning} Our translation approach starts by \emph{partitioning the Go snippet into  fragments to be translated individually}: the datatype declaration, the function definition and the method definition. These fragments are then organised into a \emph{dependency graph}, where \gocode{addendaFieldInclusion} depends on \gocode{EntryDetail} and \gocode{checkAddenda02}.

\paragraph{Type-driven translation: type compatibility checks} Next, we proceed to the type-driven translation phase. The dependency graph is traversed in postorder to translate each individual fragment: first the type declaration \gocode{EntryDetail}, then \gocode{checkAddenda02} (which is called by \gocode{addendaFieldInclusion}), and finally   
\gocode{addendaFieldInclusion}.

A possible  translation for \rustcode{EntryDetail} obtained from the LLM is given in
\autoref{fig:overview-incorrect-rust}, 
where the nullability is missing as \rustcode{Vec<Option<Box<Addenda05$>>>$} is a non-null object. If the only correctness check in this translation phase was denoted by the Rust compiler, we would ignore this fact and 
proceed to translate  \gocode{checkAddenda02}, followed by
\gocode{addendaFieldInclusion}, 
with a potential translation captured in \autoref{fig:overview-incorrect-rust}.
%
Although this translation passes the Rust compiler, it doesn't preserve the behaviour of the original code. 
In particular, the original Go method \gocode{addendaFieldInclusion} receives an argument \gocode{entry} of type \gocode{EntryDetail} and performs a null check on the \gocode{Addenda05} field: \gocode{entry.Addenda05 != nil}. Instead, \rustcode{addenda\_field\_inclusion} in the translation 
checks if any entry into \rustcode{entry.addenda05} is null: \rustcode{entry.addenda05. iter().any(|a| a.is\_some())}.

Our observation is that the root of this translation error is the fact that  the Rust translation of \rustcode{EntryDetail} is not compatible with the original Go version. Informally, we consider \emph{a translated Rust type to be compatible with the original Go type if any feasible value that can inhabit the Go type,
% (as it is used by the original project)
can also inhabit the Rust type} (we will revisit the notion of \emph{feasible value} at the end of the section).
\cd{this relation is not commutative; do we want it to be?} For our current example, 
a null value can inhabit \gocode{Addenda05}, but not \rustcode{addenda05}, 
causing the \emph{type compatibility check} to fail. Consequently, we re-query the LLM, and get the correct translation in \autoref{fig:rust_overview}, which wraps \rustcode{Option} around \rustcode{Vec}.
In addition to compatibility checks for type declarations, we also perform type compatibility checks for function/method signatures, which check the compatibility of their constituent types. For our running example, all signature compatibility checks pass once we have the correct translation of \gocode{EntryDetail}.

\paragraph{Type-driven translation: feature mapping} We next focus on the error handling in the original Go code in \autoref{fig:go_overview}, 
where both \gocode{checkAddenda02} and \gocode{addendaFieldInclusion}
return a value of type \gocode{error}.
The builtin \gocode{error} type is an \gocode{interface} type containing exactly one method: \gocode{Error() string}. Custom error types often implement this interface and are passed around as \gocode{error} rather than concrete types. Then, type assertions are used to recover the concrete underlying type. In this example,  \gocode{addendaFieldInclusion} checks whether the error returned by \gocode{checkAddenda02 } is an instance of the custom error \gocode{BatchError}: \gocode{err.(*BatchError)}.
%
Although the translation produced by the LLM for \rustcode{addenda\_field\_inclusion} in \autoref{fig:rust_overview} looks idiomatic, it does not compile due to the erroneous emulation of the syntax of the Go source: the Go type assertion \gocode{err.(*BatchError)} is translated to  \rustcode{err.downcast::<BatchError>()}, which is not a valid Rust expression.

LLMs have been found to struggle with accurately mapping features, especially when subtle syntactic or semantic differences exist between constructs in the source and target languages~\cite{yin2024rectifiercodetranslationcorrector}. In such cases, LLMs may mimic source language syntax incorrectly or misalign source APIs with target ones, resulting in code that fails to compile or diverges from the original code's behavior.

Our solution is to predefine feature mapping rules  that
map language features of the source language to the target language
in order to constrain the LLM-based translation. For error handling, we define a  unified concrete Rust error type to map \gocode{error} to. Namely, we choose \rustcode{anyhow::Error}, which is provided by a popular third party Rust library for idiomatic error handling~\cite{anyhow}. While the exact rule for 
feature mapping of error handling will be given in Section~\ref{sec:error-handling},
for now, we provide the correct translation in \autoref{fig:rust_overview}.

\paragraph{Semantics-driven translation}
\cd{finish this}
At the end of the type-driven translation phase, we obtain the \emph{type compatible project translation} in \autoref{fig:rust_overview}, 
and make the assumption that the types and function signatures are correct.
Following the same order from the type-driven phase (i.e. \rustcode{check\_addenda02} first, and \rustcode{addenda\_field\_inclusion} second), we use the unit tests to check that they maintain the semantics of their corresponding original code. To be modular, when 
checking \rustcode{addenda\_field\_inclusion}, we mock \rustcode{check\_addenda02}.


\begin{figure}[!htb]
    \centering
    \begin{minipage}{.47\textwidth}
        % \centering
        \begin{lstlisting}[language=go, basicstyle=\tiny\ttfamily,escapechar=\&]

type EntryDetail struct {
	Addenda05 []*Addenda05
}

func checkAddenda02() error { ... }

func (batch *Batch) addendaFieldInclusion(entry *EntryDetail) error {
    if entry.Addenda05 != nil {
        return batch.Error(...)
    }

    if err := checkAddenda02(); err != nil {
        if _, ok := err.(*BatchError); ok {
	       return err
        }
        return BatchError{err}
    }
    ...
}
\end{lstlisting}
        \caption{Source Go snippet}
        \label{fig:go_overview}
        \end{minipage}
    \begin{minipage}{0.5\textwidth}
        % \centering
        \begin{lstlisting}[language=rust, basicstyle=\tiny\ttfamily]
pub struct EntryDetail {
    pub addenda05: Vec<Option<Box<Addenda05>>>,
}

pub fn check_addenda02() -> Result<(), Addenda02Error> { ... }

pub fn addenda_field_inclusion(&self, entry: &EntryDetail) -> Result<(), BatchError> {
    if entry.addenda05.iter().any(|a| a.is_some()) {
        self.error(..)?;
    }
    if let Err(err) = check_addenda02() {
        if let Ok(err) = err.downcast::<BatchError>() 
        {
            return err
        }
        return BatchError(err)
    }
    ...
}
\end{lstlisting}
        \caption{Incorrect translation to Rust}
        \label{fig:overview-incorrect-rust}
    \end{minipage}%
    \end{figure}
    %\begin{minipage}{0.5\textwidth}
     %   \begin{lstlisting}[language=rust, basicstyle=\tiny\ttfamily]
%pub struct EntryDetail {
 %   pub addenda05: Vec<Option<Box<Addenda05>>>,
%}
%pub fn addenda_field_inclusion(&self, entry: &EntryDetail) -> Result<()> {
%    if entry.addenda05.iter().any(|a| a.is_some()) {
%        self.error(..)?;
%    }
%    ...
%}
%\end{lstlisting}
 %       \caption{Translated Rust snippet}
  %      \label{fig:rust_snippet_semantics}
  %  \end{minipage}

\begin{figure}[!htb]
    \centering
    \begin{minipage}{.7\textwidth}
        % \centering
        \begin{lstlisting}[language=go, basicstyle=\tiny\ttfamily]

pub struct EntryDetail {
    pub addenda05: Option<Vec<Option<Box<Addenda05>>>>,
}

pub fn check_addenda02() -> Result<(), anyhow::Error> { ... }

pub fn addenda_field_inclusion(&self, entry: &EntryDetail) -> Result<(), anyhow::Error> {
    if entry.addenda05.is_some() {
        self.error(..)?;
    }
    if let Err(err) = check_addenda02() {
        if let Ok(err) = err.root_cause().downcast::<BatchError>() 
        {
            return anyhow!(err)
        }
        return anyhow!(BatchError(err))
    }
    ...
}
\end{lstlisting}
        \caption{Correct translation to Rust}
        \label{fig:rust_overview}
        \end{minipage}
    \end{figure}


==> sections/intro_brandon.tex <==
\section{Introduction}
\bp{Could potentially cut this paragraph if need be}
Code translation 
% --- the task of translating source code in one high-level programming language to another high-level programming language --- 
has many important practical applications. For example, a developer may wish to modernize their application~\cite{modernization, developersperceive}, they may wish to maintain a client SDK in multiple languages~\cite{awssdk, googlesdk, azuresdk}, or they may wish to obtain the benefits of another language~\cite{tractor, c2rust}. The Rust language has received special attention as a target language for code translation because it achieves a strong balance between safety and performance~\cite{tractor}. However, manual code translation is tedious and error prone, hence automated code translation would save developer time and energy.

Prior work in automated translation to Rust falls into two categories: rule-based (sometimes called ``symbolic'')~\cite{c2rust, zhang2023ownership} and machine-learning (ML)-based (typically using LLMs)~\cite{tang-etal-2023-explain,RoziereLachaux2020,RoziereZhang2022,szafraniec2022code,yin2024rectifiercodetranslationcorrector}. Rule-based approaches have the advantage of being semantically correct (i.e. I/O equivalent) by construction, but often produce non-idiomatic and unmaintainable code~\cite{PanICSE24, eniser2024translatingrealworldcodellms, yang2024vertverifiedequivalentrust}. Conversely, ML-based approaches are usually more idiomatic and maintainable, but come without correctness guarantees. 

Recent efforts have combined LLM-based translation with a validation step such as running unit tests, differential fuzzing~\cite{eniser2024translatingrealworldcodellms}, or formal verification~\cite{yang2024vertverifiedequivalentrust} to ensure semantic correctness. If validation fails, a new translation is generated. However, these approaches have primarily focused on translating competitive programming-style programs or small code snippets from real-world projects and struggle with translating entire projects. This limitation arises because the context windows of many state-of-the-art LLMs are not large enough to encompass entire projects. Even when the context window suffices, the probability of errors increases exponentially with the amount of code being translated~\cite{eniser2024translatingrealworldcodellms}.

In this work, we aim to move beyond code snippet translation by designing an LLM-based translation approach capable of handling \emph{entire projects} and producing \emph{validated translations}.
A natural approach to scale to entire projects, taken by us and work parallel to ours~\cite{ibrahimzada2024repositorylevelcompositionalcodetranslation, shiraishi2024contextawarecodesegmentationctorust}, is to partition the project into smaller code fragments (e.g. functions, type definitions) that can be translated individually. We can compute a dependency graph between the fragments, and translate them in post-order, which allows us to incrementally translate and validate the semantic correctness of each translated fragment before translating the next fragment. Moreover, we can provide the LLM with context about translations of previous fragments to aid in translating the current fragment. 

However, this approach alone still struggles to reliably produce semantically correct translations. In the parallel works, the semantic checks often simply crash because they lack a principled technique for ensuring the source project's functions can be compared with the translation's functions.
In addition, when the initial translation of a code fragment is incorrect (it does not compile or semantic validation fails), the LLM will often get stuck in a repair loop attempting to fix the error. For example, making a repair often has cascading effects, creating more errors. 
% In addition, when translating to Rust, some compilation errors may be nearly impossible to repair because the source project uses multiple mutable aliases or cyclic references. 
%This can halt the progress of translation, or lead to impractically long runtimes. 

% In particular, the language features of the source language often will not have direct mappings to the target language, leading the LLM to fall into common error patterns or use inconsistent coding styles. For example, the \go{} language and \rust{} have different idioms for error handling, \go{} interfaces are structural whereas \rust{} traits are nominal, and global variables in \go{} support dynamic initialization whereas \rust{} does not.

% In addition, a given code fragment's translation may be incompatible with the previously translated fragments, e.g., there may be compilation errors, or semantic validation may fail. If we allow the LLM unrestricted ability to make modifications to the translated codebase to repair the error, it may make changes that have cascading effects on other parts of the code, leading the LLM to get stuck in a repair loop. 

%Our solution is to provide stricter guidance to the LLM in order to minimize the number of errors it makes from the outset.

In order to address this challenge, we apply two strategies.

\paragraph{\textbf{Type-Compatibility-Driven Translation}}
We draw inspiration from language interoperability~\cite{multi-language-semantics}, and define a set of criteria for \textit{type-compatibility}, which ensure that functions in the source project and translation can be compared. We then divide the translation into two-phases: a type-compatibility driven translation phase, and a semantics driven phase.

During the type-compatibility-driven phase, we translate all code fragments of the source project, during which we repair any compilation errors and ensure our type-compatibility criteria are met. Enforcing our type-compatibility criteria during this phase helps catch translation errors earlier on, whereas prior works would only catch these types of errors when they attempt to validate semantic correctness. We then move to the semantics-driven translation phase, in which we use the source projects unit tests to validate the I/O equivalence of the functions of the source project and translation. When repairing semantic validation failures, we restrict repairs to the function under test, ensuring that translation finishes in a reasonable amount of time.
% First, we propose a modular, two-phased approach to translation, which restricts the search space of repairs in a way that reduces the chance of cascading effects due to a repair, and allows us to translate a code fragment even if its dependencies could not be successfully translated. Our approach divides translation into a type-driven phase and a semantic-driven phase. 

% During the type-driven phase, we focus on getting a translation that passes Rust’s type checker (i.e. compiler), and satisfies language inter-operability criteria which ensure that unit tests from the source project can be executed directly on the translation. We define these criteria as type- and signature-compatibility. During this phase, we translate all code fragments. We allow the LLM to make arbitrary modifications to the translation to repair compiler and type/function compatibility errors, but we defer checking semantic equivalence until the next phase. When we are unable to repair errors for a given translated code fragment, we give up and create a mock translation which emulates the behavior of the code fragment. Our mocking approach makes the translation modular, in that we can translate a code fragment even if we failed to translate its dependent code fragments.

% During the semantic-driven phase, we leverage the unit tests of the source project to check for I/O equivalence between the functions/methods of the source project and translation. When testing a given function/method's translation, we mock its callees, thus ensuring that any inequivalence is caused by a bug in the given function. Moreover, we make the assumption that the types and function signatures are correct, allowing us to restrict the repair effort to just the body of the current function. This restriction reduces the search space of potential repairs and helps to ensure translation procedure terminates in a reasonable amount of time. 

\paragraph{\textbf{Hybrid Translation Rules for Translating Source Language Features}}
We find that the LLM often makes errors when translating features of the source language that do not have direct mappings to the target language. For example, the \go{} language and \rust{} have different idioms for error handling, \go{} interfaces are structural whereas \rust{} traits are nominal, and global variables in \go{} support dynamic initialization whereas \rust{} does not. Without anything to guide translation of these language features, the LLM will often make mistakes.

To prevent the LLM from repeating these common mistakes, we propose translation rules that map language features of the source language to the target language. While we could take a traditional rule-based approach by writing symbolic translation rules, such a task would require substantial effort to ensure all cases are covered, and prior work has has shown symbolic rules have difficulty producing idiomatic code. This motivates us to develop \textit{hybrid} rules wherein the translation rule is written in natural language instructions for the LLM, and then we perform static checks on the resulting translation to ensure the rules are followed. This approach is easy to implement, and produces more idiomatic code than symbolic translation rules.
\\

%Real-world \go{} projects often consist of multiple packages, with source code organized in a complex project layout.  
% The challenge arises from the different code organization principles of
% \go{} and \rust{}. A \go{} project consists of packages, where a package can span multiple files. Private items are visible to other items in the same package, even if they are not in the same file. Conversely, \rust{} obeys a module system,  where each file in a \textcolor{Rust}{cargo} project is a module. Items in a module cannot be directly used by items in another module. Relying on the LLM to make decisions on the project structure and appropriately generate import statements and amend visibility modifiers is problematic. 
% In fact, Yin et al. found that the most frequent compilation errors for code obtained through LLM-based translation are related to wrong or missing import statements~\cite{yin2024rectifiercodetranslationcorrector}.
% Our approach is to emulate the original project structure, and use a dependency analysis to statically synthesise the correct import statements and visibility modifiers. 


We implement these strategies in a translation tool called \ourtool{}. While the fundamental ideas proposed in our work are agnostic to the programming language, \ourtool{} specifically targets translating \go{} projects into \rust{} projects. We choose this language pair for several reasons. First, there is a strong push to use memory safe languages like Rust~\cite{tractor}. Second, \go{} and \rust{} operate a similar level of abstraction, and they are often used for similar tasks. Third, \rust{} offers performance and safety benefits over \go{}. Specifically, (safe) \rust{} eliminates data races, and it does not have the overhead of a runtime. Thus there is a strong argument to be made for re-writing \go{} code to \rust{}.

We evaluate \ourtool{} on three open source \go{} projects with up to 4.6K lines of code, and covering various use cases including banking transactions, statistics, and string algorithms. Our results show that the two strategies we propose enable us to reliably generate translations that pass the \rust{} compiler, and that, on average, we are able to successfully validate the I/O equivalence 63\% of the functions in the translation. We also show that both our type-compatibility checks and hybrid translation rules are critical for reliably producing translations of entire projects. These results are promising, as parallel work~\cite{ibrahimzada2024repositorylevelcompositionalcodetranslation} shows that even a partially correct translation significantly reduces developer time to translate a code base.

Our results compares favorably with this parallel work as well work~\cite{ibrahimzada2024repositorylevelcompositionalcodetranslation}, which reports successfully validating I/O equivalence of only 45\% of translated functions on average. They also report that I/O equivalence validation checks simply crash for 24.7\% of translated functions. We believe our improvement is due to our type compatibility checks, which ensure I/O equivalence validation does crash.

In summary, we make the following contributions.
\begin{itemize}
    \item We propose techniques for improving the scalability and reliability of LLM-based code translation.
    \item We propose hybrid translation rules to map features between the original and target code, thus avoid mistakes commonly made by LLMs.
    \item We propose a two-phased repair approach divided into type-driven repairs and semantic repairs that reduces the search space of repairs, and reduces the chance the LLM gets stuck in a repair loop.
    \item We implement our proposed approach in a tool \ourtool{}, and demonstrate its ability to reliably produce useful \rust{} translations on three open-source \go{} projects. 
\end{itemize}

==> sections/overview_interfaces.tex <==
\section{Overview of our approach}
%\cd{revise and use running example}
%We construct a call-graph, which we then traverse in post-order, and translate each individual function.
We illustrate our approach using the example in Figure~\ref{fig:go_overview}, which is a contrived version of code extracted from the realworld benchmark \textbf{ach}. 
%
\begin{figure}[!h]
    \centering
    \begin{minipage}{.47\textwidth}
        % \centering
        \begin{lstlisting}[language=go, basicstyle=\tiny\ttfamily,escapechar=\&]
// in file types.go
type EntryDetail struct {
	Addenda05 []*Addenda05
}

type Batch struct { ... }

// in file batch.go
func (batch *Batch) Validate(entry *EntryDetail) error {
    if entry.Addenda05 != nil {
        return batch.Error(...)
    }
    ...
}
func (batch *Batch) SetID(string id) {...}
\end{lstlisting}
        %\caption{Source Go snippet}
        %\label{fig:go_overview}
        \end{minipage}
    \begin{minipage}{0.5\textwidth}
        % \centering
        \begin{lstlisting}[language=rust, basicstyle=\tiny\ttfamily,escapechar=\&]
// in file interfaces.go
type Batcher interface {
    Validate(*EntryDetail) error
    SetID(string)
    ...
}

type canValidate interface {
    Validate(*EntryDetail) error
}    
&\newline&
&\newline&
&\newline&
&\newline&
&\newline&
&\newline&
\end{lstlisting}
        %\caption{Incorrect translation to Rust}
        %\label{fig:overview-incorrect-rust}
    \end{minipage}%
    \caption{Source Go code consisting of three files: types.go, batch.go and interfaces.go}
        \label{fig:go_overview}
    \end{figure}


The example features three files: ``types.go'' containing the declaration of types \gocode{EntryDetail} and \gocode{Batch},
``batch.go'' containing
methods
\gocode{Validate} and \gocode{SetID}, and ``interfaces.go'' defining interfaces \gocode{Batcher} and \gocode{canValidate}. 
%Go interfaces are sets of method signatures. 
The set of methods representing \gocode{canValidate} (which only contains method \gocode{Validate}) is a subset of the set denoting \gocode{Batcher}.
We assume all three files are located in the same package.

\paragraph{\textbf{Project partitioning}} Our translation approach starts by partitioning the Go code into  fragments to be translated individually: \gocode{EntryDetail},
\gocode{Batch},
\gocode{Validate},
\gocode{SetID},
\gocode{Batcher} and \gocode{canValidate}. These fragments are then organised into a \emph{dependency graph}, where the dependency relations are as follows: \gocode{Validate} depends on \gocode{EntryDetail},
\gocode{Batch},
\gocode{Batcher} and \gocode{canValidate};
\gocode{SetID} depends on
\gocode{Batch} and
\gocode{Batcher}; 
\gocode{Batcher} depends on \gocode{canValidate}.

\paragraph{\textbf{Type-driven translation: type compatibility checks}} Next, we proceed to the type-driven translation phase. The dependency graph is traversed in postorder to translate each individual fragment: first \gocode{EntryDetail}, then
\gocode{Batch},
\gocode{canValidate},
\gocode{Batcher},  
\gocode{Validate}
and finally   
\gocode{SetID}.
%
A~possible  translation for \rustcode{EntryDetail} obtained from the LLM is given in
\autoref{fig:rust_overview_wrong}.
While the Go \gocode{EntryDetail} has a nullable slice \gocode{[]*Addenda05}, the Rust 
\rustcode{Vec<Option<Box<Addenda05$>>>$} is a non-null object. If the only correctness check in this translation phase was done by the Rust compiler, we would miss this discrepancy (as it doesn't trigger a compilation error), and proceed with the rest of the translation. The only code in our example that uses \gocode{EntryDetail} and could signal the translation error is  method 
\gocode{Validate}. 
A translation obtained from the LLM for \gocode{Validate} is captured in \autoref{fig:rust_overview_wrong}, where we ignore for now the details related to traits.
%
Again, this translation doesn't raise a compilation error although it doesn't preserve the behaviour of the original code: the original Go method \gocode{Validate} receives an argument \gocode{entry} of type \gocode{EntryDetail} and performs a null check on the \gocode{Addenda05} field
(\gocode{entry.Addenda05 != nil}); instead, its translation, \rustcode{Validate},
checks if any entry into \rustcode{entry.addenda05} is null  (\rustcode{entry.addenda05.iter().any(|a| a.is\_some())}).

Our observation is that an incorrect type translation can lead the LLM to compensate by generating subsequent code that compiles (i.e. aligns with the flawed type translation), but may not preserve the original code's behavior.
Consequently, the goal of our type-driven translation phase is to detect as many type-related translation errors, as early as possible. For the particular translation errors encountered for \rustcode{EntryDetail} and \rustcode{validate} in \autoref{fig:rust_overview_wrong}, they originate from the fact that  the Rust translation of \rustcode{EntryDetail} is not compatible with the original Go version. Informally, we consider \emph{a translated Rust type to be compatible with the original Go type if any feasible value that can inhabit the Go type,
% (as it is used by the original project)
can also inhabit the Rust type} (we will revisit the notion of \emph{feasible value} at the end of the section).
\cd{this relation is not commutative; do we want it to be?} For our current example, 
a null value can inhabit \gocode{Addenda05}, but not \rustcode{addenda05}, causing the type compatibility check to fail. Note that this check takes place immediately after the translation of \gocode{EntryDetail} and it is local (i.e. it only involves the translation of \gocode{EntryDetail}). Following the failure of the compatibility check, we re-query the LLM, and obtain the correct translation \rustcode{EntryDetail}
in \autoref{fig:rust_overview_correct}, which wraps \rustcode{Option} around \rustcode{Vec}. With the correct translation \rustcode{EntryDetail}, the LLM generates the correct translation \rustcode{validate}, also given in \autoref{fig:rust_overview_correct}.

In addition to compatibility checks for type declarations, we also perform type compatibility checks for function/method signatures, which check the compatibility of their constituent types. For our running example, all signature compatibility checks pass once we have the correct translation of \gocode{EntryDetail}.

\paragraph{\textbf{Type-driven translation: feature mapping}} We next focus on the two interfaces \gocode{Batcher} and \gocode{canValidate} in the original Go code in \autoref{fig:go_overview}.
%
There are several problems with the translation in \autoref{fig:rust_overview_wrong}.
First, it fails to preserve the sub-interfacing relation between \rustcode{Batcher} and \rustcode{canValidate}. 
In particular, a Go interface is \emph{structural}, meaning that \gocode{Batcher} is automatically a sub-interface of \gocode{canValidate} due to the common method signature for \gocode{Validate}. Conversely to Go interfaces, a Rust \rustcode{trait} is \emph{nominal}, and thus the sub-interfacing relation does not hold. This is a significant translation error as, for any Go code where a value of type \gocode{Batcher} is assigned to/upcast to a variable of type \gocode{canValidate},
there won't exist any compilable Rust translation. 
Additionally, because in Rust
the concrete method implementations need to be provided explicitly in an \rustcode{impl} block, 
the implementation of the
\rustcode{validate} method needs to be duplicated, once for \rustcode{Batcher} and once for \rustcode{canValidate}. A naive approach may lead the LLM to generate different code for the two implementations of \rustcode{validate}.

The difficulty in correctly mapping Go interfaces to Rust traits highlights a broader challenge: LLMs often struggle with accurately mapping features, particularly when there are subtle syntactic or semantic differences between constructs in the source and target languages~\cite{yin2024rectifiercodetranslationcorrector}. In such cases, LLMs may mimic source language syntax incorrectly or misalign source APIs with target ones, resulting in code that fails to compile or diverges from the original code's behavior. As explained in the introduction, our solution is to predefine feature mapping rules that constrain the LLM-based translation. When mapping Go interfaces to Rust traits, we predefine a way of breaking a trait into multiple sub-traits. While the exact feature mapping rule will be given in Section~\ref{sec:interface-mapping},
for now we provide the correct translation in \autoref{fig:rust_overview_correct}.

\paragraph{\textbf{Type-driven translation: visibility modifiers}}
In the Go code shown in \autoref{fig:go_overview}, where all the files are in the same package, all items are accessible to one another due to Go's visibility rules. By contrast, Rust defaults to private visibility, where items are only accessible within the same module (i.e. file in our case). Rather than depending on the LLM, we symbolically generate the appropriate visibility modifiers for the Rust translation, as demonstrated in Figure~\ref{fig:rust_overview_correct}, where \rustcode{pub} is added to make items public where appropriate.
\paragraph{\textbf{Semantics-driven translation}}
\cd{finish this}
At the end of the type-driven translation phase, we obtain the \emph{type compatible project translation} in \autoref{fig:rust_overview}, 
and make the assumption that the types and function signatures are correct.
Following the same order from the type-driven phase (i.e. \rustcode{check\_addenda02} first, and \rustcode{addenda\_field\_inclusion} second), we use the unit tests to check that they maintain the semantics of their corresponding original code. To be modular, when 
checking \rustcode{addenda\_field\_inclusion}, we mock \rustcode{check\_addenda02}.

\paragraph{\textbf{Project layout and import statements}}



\begin{figure}[!htb]
    \centering
    \begin{minipage}{.47\textwidth}
        % \centering
        \begin{lstlisting}[language=go, basicstyle=\tiny\ttfamily,escapechar=\%]
// in file types.rs
struct EntryDetail {
    addenda05: Vec<Option<Box<Addenda05>>>,
}

struct Batch { ... }

// in file batch.rs
impl Batcher for Batch {
    fn validate(&self, entry: &EntryDetail) -> Result<()> {
        if entry.addenda05.iter().any(|a| a.is_some()) {
            self.error(..)?;
        }
        ...
    }
    fn set_id(&mut self, id: String) { ... }
    ... 
}

\end{lstlisting}
        %\caption{Source Go snippet}
        %\label{fig:go_overview}
        \end{minipage}
    \begin{minipage}{0.5\textwidth}
        % \centering
        \begin{lstlisting}[language=rust, basicstyle=\tiny\ttfamily,escapechar=\%]
// still in file batch.rs
impl canValidate for Batch {
    fn validate(&self, entry:&EntryDetail)->Result<()> 
    {
       // duplicated implementation
    }
}

// in file interfaces.rs
trait Batcher {
    fn validate(&self, entry: &EntryDetail)->
                                 Result<()>;
    fn set_id(&mut self, id :String);
    ...
}

trait canValidate {
    fn validate(&self, entry: &EntryDetail)->
                                 Result<()>;
} 
\end{lstlisting}
        %\caption{Incorrect translation to Rust}
        %\label{fig:overview-incorrect-rust}
    \end{minipage}%
    \caption{Incorrect Rust translation for the Go code in \autoref{fig:go_overview}}
        \label{fig:rust_overview_wrong}
    \end{figure}

\begin{figure}[!htb]
    \centering
    \begin{minipage}{.47\textwidth}
        % \centering
        \begin{lstlisting}[language=go, basicstyle=\tiny\ttfamily,escapechar=\%]
// in file types.rs
pub struct EntryDetail {
    pub addenda05: Option<Vec<Option<Box
                               <Addenda05>>>>,
}

struct Batch { ... }

// in file batch.rs
use crate::interfaces::{Batcher_validate};
use crate::entry_detail::EntryDetail
impl Batcher_validate for Batch {
    fn validate(&self, entry: &EntryDetail) -> Result<()> {
        if entry.addenda05.is_some() {
            self.error(..)?;
        }
        ...
    } }
\end{lstlisting}
        %\caption{Source Go snippet}
        %\label{fig:go_overview}
        \end{minipage}
    \begin{minipage}{0.5\textwidth}
        % \centering
        \begin{lstlisting}[language=rust, basicstyle=\tiny\ttfamily,escapechar=\%]
// in file interfaces.rs
pub trait Batcher_validate {
    fn validate(&self, entry: &EntryDetail) -> Result<()>;
}
pub trait Batcher_set_id {
    fn set_id(&mut self, id: String);
}
...
pub trait Batcher: Batcher_validate + Batcher_set_id + ... {}
impl<T> Batcher for T where T: Batcher_validate + Batcher_set_id + ... {}

pub(crate) trait canValidate: Batcher_validate {}
impl<T> canValidate for T where T: Batcher_validate {}
%\newline%
%\newline%
%\newline%
\end{lstlisting}
    \end{minipage}%
    \caption{Correct Rust translation for the Go code in \autoref{fig:go_overview}}
        \label{fig:rust_overview_correct}
    \end{figure}
      

==> sections/overview_simplified.tex <==
\section{Overview of our approach} \label{sec:overview}
%\cd{revise and use running example}
%We construct a call-graph, which we then traverse in post-order, and translate each individual function.
We illustrate our approach using the example in Figure~\ref{fig:go_overview}, which is a contrived version of code extracted from one of our real-world benchmarks for validating banking transactions~\cite{ach}. The example consists of three files: ``types.go'', which declares the type \gocode{EntryDetail}; ``globals.go'', which defines the global variable \gocode{specialNumber} initialized by a call to \gocode{setupSpecialNumber}; and ``validator.go'', which contains the definition of the function \gocode{Validate}.
We assume all three files are located in the same package.
%
\begin{figure}[!h]
    \centering
    \begin{minipage}{.47\textwidth}
        % \centering
        \begin{lstlisting}[language=go, basicstyle=\tiny\ttfamily,escapechar=\&]
// in file types.go
type EntryDetail struct {
	Addenda05 []int
}

&\newline&
// in file globals.go
var specialNumber int = setupSpecialNumber()

func setupSpecialNumber() int { ... }
&\newline&
&\newline&
&\newline&
&\newline&
&\newline&
\end{lstlisting}
        %\caption{Source Go snippet}
        %\label{fig:go_overview}
        \end{minipage}
    \begin{minipage}{0.5\textwidth}
        % \centering
        \begin{lstlisting}[language=rust, basicstyle=\tiny\ttfamily,escapechar=\&]
// in file validator.go        
func Validate(entry *EntryDetail, length int) bool {
    if entry.Addenda05 != nil {
        // length check
        if len(entry.Addenda05) != length {
            return false
        }
        // search for special number
        for _, r := range entry.Addenda05 {
            if r == specialNumber { return true; }
        }
        return false;
    }
    return false;
}
\end{lstlisting}
        %\caption{Incorrect translation to Rust}
        %\label{fig:overview-incorrect-rust}
\end{minipage}%
\caption{Source Go code consisting of three files: types.go, batch.go and interfaces.go}
    \label{fig:go_overview}
\end{figure}

Translation then proceeds in three phases: \textbf{project partitioning}, \textbf{type-driven translation}, and \textbf{semantics-driven translation}. 

\emph{\textbf{Project partitioning.}} 
Our approach first partitions the code into fragments to be translated individually. We create a fragment for each function/method, type definition (i.e. struct or interface), and global variable declaration. Specifically, we create fragments for: 
\gocode{EntryDetail}, \gocode{specialNumber}, \gocode{setupSpecialNumber} and \gocode{Validate}. 
These fragments are then organised into a \emph{dependency graph}, where the dependency relations are as follows: 
\gocode{specialNumber} depends on \gocode{setupSpecialNumber};
\gocode{Validate} depends on \gocode{EntryDetail} and \gocode{specialNumber}.
% \cd{draw the graph?}

\emph{\textbf{Type-driven translation: feature mapping.}} Next, we proceed to the type-driven translation phase. The dependency graph is traversed in postorder to translate each individual fragment: first 
\gocode{setupSpecialNumber},
then
\gocode{specialNumber},
\gocode{EntryDetail}
and finally   
\gocode{Validate}.
%
Let's assume we have a translation for \gocode{setupSpecialNumber}, and focus on the global variable \gocode{specialNumber}. A translation obtained from Anthropic's Claude 3 Sonnet 
for its definition is given in
\autoref{fig:rust_overview_wrong}, where the global variable definition is translated to a global \rustcode{static} definition.
%
\begin{figure}[!h]
    \centering
    \begin{minipage}{.47\textwidth}
        % \centering
        \begin{lstlisting}[language=rust, basicstyle=\tiny\ttfamily,escapechar=\%]
// in file types.rs
struct EntryDetail {
    addenda05: Vec<i32>,
}

%\newline%
// in file globals.rs
static special_number: i32 = setup_special_number()

fn setup_special_number() -> int { ... }
%\newline%
%\newline%
%\newline%
%\newline%
%\newline%
\end{lstlisting}
        %\caption{Source Go snippet}
        %\label{fig:go_overview}
        \end{minipage}
    \begin{minipage}{0.5\textwidth}
        % \centering
        \begin{lstlisting}[language=rust, basicstyle=\tiny\ttfamily,escapechar=\%]
// in file validator.rs        
fn validate(length: u32, entry: &EntryDetail)->bool {
    if entry.addenda05.iter().all(|x| *x!=0) {
        // length check
        if entry.addenda05.len() != length as usize {
            return false
        }
        // search for special number
        for r in entry.addenda05.iter() {
            if r == special_number return true
        }
        return false
    }
    return false
}
\end{lstlisting}
        %\caption{Incorrect translation to Rust}
        %\label{fig:overview-incorrect-rust}
    \end{minipage}%
    \caption{Incorrect Rust translation for the Go code in \autoref{fig:go_overview}}
        \label{fig:rust_overview_wrong}
    \end{figure}
%
While this may seem like an intuitive translation, it will trigger a compilation error because, while  
a \texttt{\color{Go}var} in Go can be initialized by arbitrary functions, \texttt{\color{Rust}static} in Rust can only initialized by \emph{const functions} (i.e. functions that can be evaluated at compile-time). 

The difficulty in correctly mapping Go global variable definitions to a Rust one highlights a broader challenge: LLMs often struggle with accurately mapping features, particularly when there are subtle syntactic or semantic differences between constructs in the source and target languages~\cite{yin2024rectifiercodetranslationcorrector}. In such cases, LLMs may mimic source language syntax incorrectly or misalign source APIs with target ones, resulting in code that fails to compile or diverges from the original code's behavior. 

As outlined in the introduction, our solution involves using predefined feature mapping rules to constrain the LLM-based translation. These rules are tailored to a specific pair of source and target languages. %When a feature in the source language can be mapped to the target language in multiple ways, feature mapping allows developers to select their preferred mapping and ensures its consistent application throughout the translation process. 
%
For the particular case of global variable definition, 
several workarounds are available, utilising constructs like \texttt{\color{Rust}Lazy} and \texttt{\color{Rust}lazy\_statics}, which defer function evaluation until its first access.
We pick the former option, and instruct the LLM on the desired target feature. Consequently, Claude 3 generates
the correct translation for \gocode{special\_number} shown in \autoref{fig:rust_overview_correct}.
%  
\begin{figure}[!h]
    \centering
    \begin{minipage}{.47\textwidth}
        % \centering
        \begin{lstlisting}[language=rust, basicstyle=\tiny\ttfamily,escapechar=\%]
// in file types.rs
pub struct EntryDetail {
    addenda05: Option<Vec<i32>>,
}
// in file globals.rs
static special_number: Lazy<i32> =
        Lazy::new(|| setup_special_number())
fn setup_special_number() -> int { ... }
\end{lstlisting}
        %\caption{Source Go snippet}
        %\label{fig:go_overview}
        \end{minipage}
    \begin{minipage}{0.5\textwidth}
        % \centering
        \begin{lstlisting}[language=rust, basicstyle=\tiny\ttfamily,escapechar=\%]
// in file validator.rs        
use crate::types::EntryDetail;
use crate::globals::special_number;
fn validate(entry: &EntryDetail, length: u32)->bool {
    if entry.addenda05.is_some() {
        // same as %\autoref{fig:rust_overview_wrong}%
        ...
%\newline%
\end{lstlisting}
    \end{minipage}%
    \caption{Correct Rust translation for the Go code in \autoref{fig:go_overview}}
        \label{fig:rust_overview_correct}
    \end{figure}
      
\emph{\textbf{Type-driven translation: type compatibility checks.}}
After correctly translating the global variable definition \rustcode{special\_number} as described earlier, the Rust translation in \autoref{fig:rust_overview_wrong} compiles successfully. However, some errors remain. Notably, in the original Go code, the \gocode{Addenda05} field of \gocode{EntryDetail} can be null, whereas in the Rust translation, the corresponding field \rustcode{addenda05} is of type \rustcode{Vec<i64>}, which implies a non-nullable object.
%
This translation error does not trigger a compilation issue because, when translating the body of \gocode{Validate}, the LLM prioritised creating code that compiles (aligning with the erroneous type \rustcode{EntryDetail}) over maintaining semantic equivalence. Specifically, the original Go method \gocode{Validate} performs a null check on the \gocode{Addenda05} field of the \gocode{entry} argument (i.e. \gocode{entry.Addenda05 != nil}), whereas its Rust translation, \rustcode{validate}, incorrectly checks if all values in \rustcode{entry.addenda05} are non-zero (i.e. \rustcode{entry.addenda05.iter().all(|x| *x!=0)}). More broadly, we observed that an incorrectly translated type can have lasting negative effects on subsequent translations, as the LLM tends to prioritise generating code that compiles with the erroneous type over ensuring semantic correctness.

The goal of our type-driven translation phase is to catch type translation errors, including those that might otherwise be overlooked by the Rust compiler. The specific errors seen for \rustcode{EntryDetail} and \rustcode{validate} in \autoref{fig:rust_overview_wrong} stem from the incompatibility between the Rust translation of \gocode{EntryDetail} and its original Go version. Informally, we consider \emph{a translated Rust type to be compatible with the original Go type if any feasible value that can inhabit the Go type,
can also inhabit the Rust type}. 
For our current example, a null value can inhabit \gocode{Addenda05}, but not \rustcode{addenda05}, causing the type compatibility check to fail. Note that this check takes place immediately after the translation of \gocode{EntryDetail} and it is local (i.e. it only involves the translation of \gocode{EntryDetail}). Following the failure of the compatibility check, we re-query the LLM, and obtain the correct translation \rustcode{EntryDetail}
in \autoref{fig:rust_overview_correct}, which wraps \rustcode{Option} around \rustcode{Vec}. 

\emph{\textbf{Type-driven translation: type compatibility checks for function signatures.}}
In addition to compatibility checks for type declarations, we also perform type compatibility checks for function/method signatures, which check the compatibility of their constituent types. For our current example, the signature of \gocode{Validate} is not compatible with the signature of its Rust translation \rustcode{validate}, where the two arguments are swapped. In particular, the signature compatibility checks fails because, with the given order, the argument types are not compatible. After re-querying, Claude 3 returns the correct translation in \autoref{fig:rust_overview_correct}. Having a dedicated type compatibility check that catches this type of errors is very important because, as explained above, these errors may escape the compiler. Additionally, when using dynamic checks to verify semantic equivalence with the original code, such type translation errors cause runtime exceptions, which are difficult to diagnose.

\emph{\textbf{Visibility modifiers and import statements.}} As noted in the introduction, LLMs often struggle to generate accurate visibility modifiers and import statements when the organisational principles of the source and target languages differ. To address this, we use a dependency analysis to post-process all translations, ensuring the correct visibility modifiers and import statements are applied, as demonstrated in~\autoref{fig:rust_overview_correct} (this is, of course, done before the compilation check). 

%\paragraph{\textbf{Visibility modifiers and import statements}}
%In the Go code shown in \autoref{fig:go_overview}, where all the files are in the same package, all items are accessible to one another due to Go's visibility rules. By contrast, Rust defaults to private visibility, where items are only accessible within the same module (i.e. file in our case). Rather than depending on the LLM, we symbolically generate the appropriate visibility modifiers for the Rust translation, as demonstrated in Figure~\ref{fig:rust_overview_correct}, where \rustcode{pub} is added to make items public where appropriate.

\emph{\textbf{Semantics-driven translation.}}
At the end of the type-driven translation phase, we obtain the \emph{type-compatible project translation} shown in \autoref{fig:rust_overview_correct}. We then proceed under the assumption that the types and function signatures are correct. Using the same order as in the type-driven phase, we check semantic equivalence of each translated global definition and each function (as we will explain later, we make use of unit tests for this purpose). To facilitate modular semantic validation, we use mocks for all callees during function checks, emulating the behavior of the source code. In this example, the translation successfully passes the semantic validation checks.


